Galton-Watson processes and their role as building blocks for branching processes

This article is an essay, both expository and argumentative, on the Galton-Watson process as a tool in the domain of Branching Processes. It is at the same time the author's ways to honour two distinguished scientists in this domain, both from the Russian Academy of Science, and to congratulate them for their special birthdays coming up very soon. The thread of the article is the role, which the Galton-Watson process had played in the author's own research. We start with an article on a controlled Galton-Watson process. Then we pass to random absorbing processes, and also recall and discuss a problem in medicine. Further questions will bring us via the Borel-Cantelli Lemma to $\varphi$-branching processes and extensions. To gain more generality, we then look at bisexual Galton-Watson processes. Finally we briefly discuss relatively complicated resource dependent branching processes to show that, here again, using Galton-Watson reproduction schemes (whenever reasonable) can be a convincing approach to new processes which are then sufficiently tractable to obtain results of interest. Keywords: Controlled branching process; $\varphi$-branching process, Bisexual reproduction, Borel-Cantelli Lemma; Resource dependence; Society forms, Stopping times, Theorem of envelopment, BRS-inequality.

==> AbstractBruss.tex <==
This article is an essay, both expository and argumentative, on the Galton-Watson process as a tool in the domain of Branching Processes.  It is at the same time the author's ways to honour two distinguished scientists in this domain, both from the Russian Academy of Science, and to congratulate them for their special birthdays coming up very soon.

The thread of the article is the role, which the Galton-Watson process had played in the author's own research.  
We start with an article on a controlled  Galton-Watson process. Then we pass to random absorbing processes, and also recall and discuss a problem in medicine. Further questions will bring us via the Borel-Cantelli Lemma
to $\varphi$-branching processes and extensions. To gain more generality, we then look at bisexual Galton-Watson processes. Finally we briefly discuss relatively complicated resource dependent branching processes to show that, here again, using Galton-Watson reproduction schemes (whenever reasonable) can be a convincing approach to new processes which are then sufficiently tractable to obtain results of interest.

\medskip
\noindent {\bf Keywords} Controlled branching process; $\varphi$-branching process, Bisexual reproduction, Borel-Cantelli Lemma; Resource dependence; Society forms, Stopping times, Theorem of envelopment, BRS-inequality.

\smallskip\noindent
{\bf Math. Subj. Index:} Primary 69J85, 60J05; secondary 60G40.
